Flag Aggregator: Scalable Distributed Training under Failures and Augmented Losses using Convex Optimization

Modern ML applications increasingly rely on complex deep learning models and large datasets. There has been an exponential growth in the amount of computation needed to train the largest models. Therefore, to scale computation and data, these models are inevitably trained in a distributed manner in clusters of nodes, and their updates are aggregated before being applied to the model. However, a distributed setup is prone to Byzantine failures of individual nodes, components, and software. With data augmentation added to these settings, there is a critical need for robust and efficient aggregation systems. We define the quality of workers as reconstruction ratios $\in (0,1]$, and formulate aggregation as a Maximum Likelihood Estimation procedure using Beta densities. We show that the Regularized form of log-likelihood wrt subspace can be approximately solved using iterative least squares solver, and provide convergence guarantees using recent Convex Optimization landscape results. Our empirical findings demonstrate that our approach significantly enhances the robustness of state-of-the-art Byzantine resilient aggregators. We evaluate our method in a distributed setup with a parameter server, and show simultaneous improvements in communication efficiency and accuracy across various tasks. The code is publicly available at https://github.com/hamidralmasi/FlagAggregator

==> authorResponse/aistats2023_author_response.tex <==
% \documentclass{article}

% \usepackage{aistats2023_author_response}
% % \usepackage{aistats-mod}
% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % define colors in text
% \usepackage{xspace}         % fix spacing around commands
% \usepackage{comment}
% \usepackage{graphicx}
% \usepackage{wrapfig}
% \usepackage{caption}
% \usepackage{subcaption}

% \begin{document}

\textbf{General Response.} {We thank the reviewers for their insightful feedback on the technical aspects of our submission and the criticism that will improve the overall strength of the paper.}
%{\color{red}We thank reviewers for their insightful comments on the technical pieces, and criticism regarding various aspects of the paper.(modify, reads meh)} 
We are glad that all reviewers found that the manuscript was well written/structured, and that our proposed Flag Aggregator (FA) to be a sensible, mathematically well-defined way to combine gradients while training deep networks in  {\bf\em noisy} distributed settings. We believe that the overall score was low due to minor conceptual, and specific novelty concerns regarding FA over existing Byzantine tolerant aggregation schemes, {especially in large-scale settings}. We will now provide answers to all such concerns, and incorporate them in the final manuscript. We hope that this will lead to a more enthusiastic support for our submission. 

%\textbf{Specific Questions:} 

% \textbf{[R1] What is Flag Median estimator for subspace?} In essence, Flag Median is an extension of the median in one-dimensional vector spaces to {\bf\em different} finite dimensional subspaces using the so-called { chordal} distance between them. From the optimization point of view, this makes the computational problem easier because {\em squared} chordal distance is smooth everywhere whereas other natural distances such as geodesic  may not be, thus slow convergence. 

% \textbf{[R1] Why is FM-based FA important and needs to be proposed for distributed optimization?} First, our hypothesis is that the true gradient lies in the subspace spanned by the clean gradients which is nicely captured by the optimization-based FM framework in (1) by $Y$. Second, in (practical) distributed settings, the quality (or noise level) of gradients in each worker may be different, {\bf and/or} each worker may use a different batch size. In such cases, handcrafted aggregation schemes may be difficult to maintain, and fine-tune. Our FM-based FA scheme can easily handle these scenarios -- we can simply reweigh gradients of worker $i$ according to its noise level before projecting onto real Stiefel manifold, {\bf and/or} use $x_i\in\mathbb{R}^{n\times b_i}$ where $b_i$ is the batch size of $i-$th worker in formulation (1). %but remain constant over (some) period of training time. In such settings, solving for the optimal solution $Y^*$ of (1) for some iterations immediately provides an easy way to identify these workers -- after which we can have simpler averaging mechanisms.  

% \textbf{[R1] Why all existing robust aggregation methods are insufficient to address the challenges considered in the manuscript?} The key challenge in handling noise in gradients is when it is dependent. Most existing methods rely just on (functions of) pairwise distances to filter gradients from workers. While this may be a good strategy when the noise in samples/gradients is independent, our experiments show that these methods are suboptimal when the noise is dependent, leading to slow convergence of the overall training procedure. For example, if all images are corrupted at fixed (but arbitrary) pixels, or permutation as in Cat Map, then the gradients may have dependent noise,  and this specific type of noise models have been increasingly used for speeding up training/finetuning networks.

% \textbf{[R1] Why the considered pairwise vectors are crucial and could be a remedy?}
% \begin{figure}[h]
% \centering
%     \includegraphics[width=0.33\linewidth]{authorResponse/figures/AuthorResponse_PairwiseCurves_CIFAR10.png}
%     \caption{CIFAR10 with ResNet-18, $n=7$, and $f=1$}
%     \label{fig:response_pairwise_gap}
% \end{figure}
% We did not intend to convey that pairwise vectors are crucial  -- this was proposed by Bulyan et al.. Under (1), we provide intuition on how FA extends Bulyan for aggregation purposes in cases where pairwise distances are useful. {In the right Figure we can see how FA improves (or similar to) Bulyan for a range of $\lambda$ in CIFAR10 with ResNet-18, $n=7$, and $f=1$.} We will clarify, and rephrase.

\textbf{[R1] What is the theoretical guarantee for the byzantine robust optimization?} Since our FA scheme is based on convexity, it is possible  to show worst-case robustness guarantees for  FA iterations under mild technical conditions on $Y^*$ -- even under correlated noise, see  for e.g. Assumption 1 in arXiv:1412.8132 (Robust Matrix Completion).

\textbf{[R1] What are the assumptions for the threat model?} Specific threat models are described under Sec 3.2, under different data augmentation routines. R1 will see that since the augmented samples are deterministic, albeit nonlinear functions of training samples, the ``noise'' is dependent across samples. Moreover, in Sec 3.3 we  also consider the effect of having unreliable communication channels with a certain drop percentage, which is common in distributed settings.
% \begin{figure}
% \centering
%     \includegraphics[width=0.33\linewidth]{authorResponse/figures/AuthorResponse_Scalability_MNIST.png}
%     \caption{MNIST with $n=60$ and $f=14$}
%     \label{fig:response_scalability}
% \end{figure}
% \textbf{[R1, R2, R4] Are the findings applicable in real-world situations with more workers?}
% We agree in distributed ML, $n$ and $f$ are usually large. To test  high-dimensional settings commonly dealt in Semantic Vision with our FA, we used ResNet-18 in submission. Now, to test the scalability of FA, we set up $n=60$ workers ($f=14$ byzantine) with MNIST dataset and a simple CNN (useful for simple detection). The right Figure shows evidence that FA is feasible to larger setups for MNIST with $n=60$, and $f=14$, and also robust with respect to choice of $\lambda$ during training. 

\textbf{1. [R4] Are the assumptions made in Lemma 1 too stringent? 2. [R2] Does FA come with convergence? 3. [R4]  Wall clock time for all figures is not provided.} 1. We make standard assumption in optimization literature -- in fact, since the feasible set of $Y$ in (1) is bounded,  assumption is satisfied. 2. Yes! In low noise settings, the average gradient is $\epsilon-$ optimal solution to FA (1) -- convergence guaranteed. 3. We apologize. We included the wall clock time for two different batch sizes in Figure 8 -- relative order between FA/baselines stays the same throughout the epochs, so we omitted. We will provide all of them in the Supplement.

%\textbf{[R4]  Wall clock time for all figures are not provided.} We apologize. We included the wall clock time with respect to epochs for two different batch sizes in Figure 8. We found that  the relative order of wall clock times stays almost the same as reported throughout the epochs, so we omitted. We are happy to provide them.



\textbf{[R2] Should the paper discuss convergence of the overall distributed training?}

Theoretical analysis of the overall distributed optimization convergence is not the focus of our paper.

\textbf{[R1] Are the results reproducible?}

We have attached the code for running the experiments and reproducing the results to our supplement submission and have mentioned this in the supplement. The majority of the reviewers have found the results reproducible.

\textbf{[R1] Does the paper explicitly and clearly state the main assumptions and limitations of the work?}

We believe that the main assumptions and limitations/details are stated in the main paper/supplement. The majority of reviewers have found this to be true.

\textbf{[R1, R5] Does the paper discuss the societal impact of the work including the impact that may arise from the misuse of the paper’s contribution?}

We do not foresee societal misuse of our contributions to robust gradient aggregation.

% \end{document}
